Karhunen Lo\`eve Expansions of Hilbert Space-Valued Random Elements

The Karhunen-Lo\`eve Expansion (KLE) of a stochastic process is a well understood eigenfunction expansion used widely in time series analysis, stochastic PDEs, and signal processing. Karhunen-Lo\`eve expansions have also been proven to exist for other types of stochastic elements whose values lie in certain $L^2$ spaces. This article provides a concise proof about the necessary and sufficient conditions for a function $v$ defined on some sample space $\Omega$ and whose values lie in some Hilbert space $\mathcal H$ to admit an eigenfunction expansion like the well-known KLE. We draw on the existing theory of Bochner spaces and Hilbert-Schmidt spaces and construct an isomorphism between them. Furthermore, this isomorphism is natural, which has important computational consequences. Finally, we demonstrate with an example the computational advantages conferred by considering the KLE in this generalized setting.

==> H-valued_functions/Introduction.tex <==


The task of binary classification involves classifying an object into one of two classes based on a list of numeric quantities associated with that object. In this thesis, we label the classes $\mathbf A$ and $\mathbf B$. For data sets where the latent feature dimension $F$ greatly exceeds the total sample size $N$, this task becomes computationally expensive and infeasible as the number of available samples for machine training may be limited. Principal component analysis and LASSO feature selection are common methods of dimension reduction to mitigate the cost of machine training on high-dimensional data sets while still ensuring that sample data are still reliably classified. 

In the asymptotic case where the latent feature dimension $F \to \infty$, we may identify each sample with a sequence $\ell_2(\N)$ or, more commonly, a function in $L^2([a,b])$\footnote{$L^2([a,b])$ denotes the Hilbert space of square-summable, Lebesgue-measurable functions $f:[a,b] \to \R$. Functions which agree a.e. are identified.}. In the same way that samples of an $F$-dimensional data set are modeled as instantiations of a Borel-measurable function $v:\Omega \to \R^F$, where the triple $(\Omega, \mathcal F, \mathbb P)$ constitutes a complete probability space, we may, in the asymptotic case $F \to \infty$, model samples as instantiations of a Borel-measurable function $v:\Omega \to L^2([a,b])$. Methods for analyzing, constructing machines from, and making predictions based off data of this nature are collectively referred to as functional data analysis (fda). %Some instances favor a fda approach, particularly when $F$ greatly exceeds the number of available samples $N$. For example, Bickel and Levine  observe a situation in which linear discriminant analysis is significantly outperformed by the much simpler naive Bayesian classification \cite{Naive Bayes}.

If we encode samples as functions in $L^2([a,b])$ One of the most useful results of fda is the existence of the \textit{KL expansion} for a Borel-measurable function $v:\Omega \to L^2([a,b])$. If $$\intp{\|v(\omega)\|_{L^2([a,b])}^2} = \intp{ \int_a^b v(\omega, x)^2 dx} < \infty$$ then $v$ admits the expansion 

\begin{equation} \label{KL expansion in L2ab}
v(x,\omega) = \E(v) + \sum_{r=1}^R \lambda_r^{1/2} Y_r(\omega) \phi_r(x)
\end{equation} 

where $R \in \N \cup \aleph_0$, $\bset{\lambda_r}_{r =1}^R$ is a non-increasing sequence of positive real numbers with \\ $\D \sum_{r = 1}^R \lambda_r = \intp{ \D \int_a^b |v(x,\omega)|^2 dx \;}$. $\bset{Y_r(\omega)}_{r=1}^R$ is an orthonormal set in the space\footnote{If $(\Omega, \mathcal F, \mathbb P)$ denotes a complete probability space, $L^2(\Omega)$ refers to the set of measurable, square-summable functions $\Omega \to \R$. Functions which agree almost surely are identified.
This is a Hilbert space over $\R$ endowed with the inner product $\aset{u, v}_{L^2(\Omega)} := \intp{u(\omega)v(\omega)} $
} $L^2(\Omega)$ and $\bset{\phi_r(x)}_{r=1}^R$ is an orthonormal set in $L^2([a,b])$. The proof of this expansion utilizes Mercer's theorem for the positive-definite, symmetric continuous kernel function $K_v:[a,b] \times [a,b] \to \R$ given by 

$$K_v(x,y) = \intp{ [v(x,\omega) - \E(v(x,\omega))][v(y,\omega) - \E(v(y,\omega))] }$$

The $\phi_r(x)$ play a role similar to that of the principal components in the case of $\R^F$ data for dimension reduction. The $\phi_r(x)$ are exactly the eigenfunctions of the operator $f \mapsto \aset{K(x,\cdot), f(x)}_{L^2([a,b])}$. Furthermore, out of all subspaces $S$ of dimension $M$ of $L^2([a,b])$, the subspace for which the mean squared error $\intp{ \|(\id - \mathbf P_S)v(x,\omega)\|^2_{L^2([a,b])} }$ is minimized is given by $\Span{\phi_r(x)}_{r=1}^M$. Throughout, $\mathbf P_S$ denotes the projection onto $S$ operator. 



It was demonstrated in \cite{KL for vector valued L2 function} that a similar expansion exists for $v: \Omega \to L^2(U, \R^P)$\footnote{For $U$ an open subset of $\R^n$ $L^2(U,\R^F)$ denotes the Hilbert space of functions $f: U \to \R^F$ for which $\int_U \|f(x)\|_{\R^F}^2 dx < \infty$. Functions which agree a.e. are identified.}. Instead, the $\phi_r(x)$ present in \eqref{KL expansion in L2ab} are an orthonormal set in $L^2(U, \R^F)$. We abstract even further, and provide a proof of a KL-like expansion for a random element $v$ in an arbitrary Hilbert space $\mathcal H$, allowing the analyst to not only abstract to the case where $F \to \infty$, but even to the case where $\mathcal H$ is not necessarily separable. 

The utility of the KL-expansion of such a $v$ lies in the way the data $\bset{\lambda_r, Y_r, \phi_r}_{r=1}^R$ can be used to construct a \textit{stochastic feature transformation}. By a stochastic feature transformation, we mean a map from some native space, (in our case, a suitable Hilbert space $\mathcal H$) to some target space (in our case $\R^{M_{res}}$ for some $M_{res} < \dim(\mathcal H))$. Typically the intent is that such a feature transformation ensures that the resulting samples in the target space exhibit the same or better separation than in the native space. We've mentioned PCA and LASSO feature selection as two examples of stochastic feature transformation. These two methods of stochastic feature transformation work by finding a map $T$ out of some class of admissible maps $\mathscr T$ such that the image of $T$ is of lower dimension 
than the domain of $T$. 

PCA, LASSO, and other methods of stochastic feature transformation should be distinguished between binary classifiers, which are  functions (or more accurately, methods for estimating functions) from some space to $\bset{0,1}$,  factoring through an indicator $\mathbb I_{(-\infty, t]}$ for some separatrix $t \in \R$. These include linear and quadratic discriminant analysis, support vector machines, LogitBoosting, RUSBoosting, and BAGging. Stochastic feature transformations are often used in conjunction with binary classifiers to elevate classification performance metrics. Our focus in this thesis is developing the theory behind the usage of the KL-expansion in constructing stochastic feature transformations from the native space $\mathcal H$ to a lower-dimensional target space and validating its efficacy with several experimental results on biomedical data sets. In particular, we cover the following points 

\begin{enumerate}
    \item We summarize a KL-expansion based stochastic feature transformation spearheaded by Castrillon and detailed in [insert sources] and []. Briefly, samples are treated as realizations of $v: \Omega \to L^2(U)$ for a simplicial complex $U$. As the stochastic feature transformation involves the construction of a nested sequence of orthogonal subspaces whose union is $L^2(U)$. We refer to this method as MLS for \textit{Multilevel Subspaces}. We detail this method in \ref{A Brief Review of MLS}

    \item We refine the MLS algorithm for stochastic feature transformation by incorporating the structure of both Class $\mathbf A$, the \textit{nominal class} and Class $\mathbf B$, the \textit{anomalous class}. In contrast, the MLS algorithm only explicitly considers the nominal class $\mathbf A$ in its construction of the stochastic feature transformation. We refer to this refined method as ACA, for \textit{anomalous class adapted}. We detail this method in section \ref{Class Concentration Bounds}
\end{enumerate}


==> H-valued_functions/Necessity.tex <==
\subsection{Necessity of The Space $L^2(\Omega, \mathcal H)$}

Theorem \ref{v has a KL expansion} demonstrates that in order for $v: \Omega \to \mathcal H$ to possess a KL expansion, $v$ must be (a representative of an equivalence class) in $L^2(\Omega, \mathcal H)$. We demonstrate that this condition is also necessary. We begin by supposing that $v$ can be represented as an $\|\cdot\|_{L^2(\Omega, \mathcal H)}$-convergent sum of the form $v = \mu + \D \sum_{r=1}^R \lambda_r Y_r \phi_r$ obeying Properties 1-5 in Definition \ref{Definition of KL expansion of v}.  

==> H-valued_functions/The_Covariance_Operator.tex <==
\subsection{The Covariance Operator} \label{The Covariance Operator}

Let $\iota: \text{HS}(\mathcal H, L^2(\Omega)) \to L^2(\Omega, \mathcal H)$ be the isometry as described in Theorem \ref{Density of HS in Bochner}. Given $v \in L^2(\Omega, \mathcal H)$, let $v_0 = v - \E(v)$ and let $H_{v_0} = \iota^{-1}(v_0)$. It follows that $\bset{\lambda_r^{1/2}}_{r=1}^R$ is the sequence of singular values of $H_{v_0}$, $\bset{\phi_r}_{r=1}^R$ is the sequence of right singular vectors of $H_{v_0}$, and $\bset{Y_r}_{r=1}^R$ is the sequence of left singular vectors of $H_{v_0}$. We may occasionally abuse notation and speak of $\bset{\lambda_r^{1/2}}_{r=1}^R$, $\bset{\phi_r}_{r=1}^R$, and $\bset{Y_r}_{r=1}^R$ as the singular values, right singular vectors, and left singular vectors respectively of $v$, rather than $H_{v_0}$, the latter being more correct. 

 Since the KL expansion of $v \in L^2(\Omega, \mathcal H)$ is formed by an SVD, we have the following properties, which will be crucial for constructing stochastic feature transformations: 

\begin{proposition}
    Let $v \in L^2(\Omega, \mathcal H)$ and let $v_0 := v - \E(v)$. For each natural number $M$, let $\mathcal A_M = \Span{\phi_r}_{r=1}^M \subseteq \mathcal H$. Then 

    \begin{enumerate}
        \item $\|v_0\|^2_{L^2(\Omega, \mathcal H)} = \D \sum_{r=1}^R \lambda_r$ 

        \item $\D \|(\id_\mathcal H - \mathbf P_S)v_0\|^2_{L^2(\Omega, \mathcal H)} \geq \|(\id_\mathcal H - \mathbf P_{\mathcal A_M})v_0\|^2_{L^2(\Omega, \mathcal H)} = \sum_{r > M} \lambda_r$ for any $\mathcal S \subseteq \mathcal H$ of dimension $M$. 
    \end{enumerate}
\end{proposition}

 We define the \textit{covariance operator} of $v$, denoted $\Cov(v)$ by $H_{v - \E(v)}^* H_{v - \E(v)}$. Immediately, the sequence $\bset{\lambda_r}_{r=1}^R$ and $\bset{\phi_r}_{r=1}^R$ comprise the descending eigenvalues and eigenvectors respectively of $\Cov(v)$. For computational purposes, it will be desirable to express $H_{v_0}$, and by extension $\Cov(v)$ without first expanding $v$ in a, potentially infinite, tensor product expansion. In fact, we see that $H_{v_0} : \mathcal H \to L^2(\Omega)$ is given by $H_{v_0}x =  \aset{v_0,x}_\mathcal H$. We can see this by simply writing $v_0$ as $\D \sum_{n=1}^N X_ne_n$, $X_n \in L^2(\Omega)$, $e_n \in \mathcal H$, $N \in \N \cup \bset{\aleph_0}$. We have for any $x \in \mathcal H$

\begin{align*}
    H_{v_0}x &= \iota^{-1}(v_0)x
        \\&=
     \sum_{n=1}^N (X_n \otimes e_n)x
    \\&=
      \aset{ \sum_{n=1}^N X_ne_n, x}_\mathcal H
     \\&=
    \aset{v,x}_\mathcal H
\end{align*}

Immediately, we have $\Cov(v)x = \E( \aset{v_0, x} v_0)$
 

==> H-valued_functions/The_Utility_of_Arbitrary_Hilbert_spaces.tex <==
\subsection{The Utility of an Arbitrary $\mathcal H$}

Because all realized data is either inherently finite, or must be sampled at a finite number of points, one may question if it is even necessary to develop the theory of the KL expansion for an arbitrary $\mathcal H$. We argue yes. 

Audio data for example, consists of a list of numbers describing the amplitude of a sound wave at equally spaced points in time. Although each audio sample necessarily contains a finite number of amplitudes, each sample can have arbitrarily many points. Thus, each can be embedded in $\ell_2(\N)$ (or $\ell_2(\N) \otimes \R^n$ in the case of $n$-channel audio). 

Image data is also well suited to infinite-dimensional $\mathcal H$. Although images contain a finite number of pixels, image resolution can be arbitrarily large. For grayscale data, an appropriate Hilbert space might be $L^2(U)$, where $U = [0,1] \times [0,1]$ If the image in question has pixel resolution $m \times n$, then it can be represented by the function 

$$f(x) = \sum_{j=1}^m \sum_{k=1}^n a_{jk} \mathbb I_{E_{jk}}(x)$$

where $E_{jk} = [\frac{j-1}{m}, \frac j m] \times [\frac{k-1}{n}, \frac k n]$  and $a_{jk}$ is the pixel intensity of the $(j,k)$-th pixel. For images whose pixels have several channel intensities (such as those with color and/or transparency data), a suitable Hilbert space is $L^2(U, \R^n) \cong L^2(U) \otimes \R^n$. 

The last utility is that one might want control of the actual inner product used on the space $\mathcal H$. 

==> Previous_Work.tex <==
\section{Previous Work}

\parencite{Santoro2023} produces a KL expansion for an element of $L^2(\Omega, \mathcal H)$ where $\Omega$ is a compact Euclidean domain (presumably with $\mathcal F = $  the $\sigma$-algebra of Lebesgue measurable sets and $\mathbb P = $ the Lebesgue measure), focusing on the conditions that . $\mathcal H$ is assumed to be separable.  



\parencite{bay2017} makes a generalization to Gaussian measures on (the norm-induced Borel $\sigma$ algebra of) separable Banach spaces. While $\mathbb P \circ v^{-1}$ constitutes a Borel measure on $\mathcal H$, we needn't assume it's Gaussian, nor must we assume $\mathcal H$ per se is separable.




